PIMSAB: A Processing-In-Memory System with Spatially-Aware Communication and Bit-Serial-Aware Computation

Bit-serial Processing-In-Memory (PIM) is an attractive paradigm for accelerator architectures, for parallel workloads such as Deep Learning (DL), because of its capability to achieve massive data parallelism at a low area overhead and provide orders-of-magnitude data movement savings by moving computational resources closer to the data. While many PIM architectures have been proposed, improvements are needed in communicating intermediate results to consumer kernels, for communication between tiles at scale, for reduction operations, and for efficiently performing bit-serial operations with constants. We present PIMSAB, a scalable architecture that provides spatially aware communication network for efficient intra-tile and inter-tile data movement and provides efficient computation support for generally inefficient bit-serial compute patterns. Our architecture consists of a massive hierarchical array of compute-enabled SRAMs (CRAMs) and is codesigned with a compiler to achieve high utilization. The key novelties of our architecture are: (1) providing efficient support for spatially-aware communication by providing local H-tree network for reductions, by adding explicit hardware for shuffling operands, and by deploying systolic broadcasting, and (2) taking advantage of the divisible nature of bit-serial computations through adaptive precision, bit-slicing and efficient handling of constant operations. When compared against a similarly provisioned modern Tensor Core GPU (NVIDIA A100), across common DL kernels and an end-to-end DL network (Resnet18), PIMSAB outperforms the GPU by 3x, and reduces energy by 4.2x. We compare PIMSAB with similarly provisioned state-of-the-art SRAM PIM (Duality Cache) and DRAM PIM (SIMDRAM) and observe a speedup of 3.7x and 3.88x respectively.

==> 50-impl.tex <==
\section{Implementation} \label{sec:implementation}



\begin{comment}
    


\subsection{CRAM Implementation}

Frequency overhead
* Doing read, compute, write in 1 cycle


Area overhead
* Sense amplifiers and write drivers
* Processing elements

\end{comment}

==> old/old-intro.tex <==
The memory latency and bandwidth stay relatively still
comparing against the exponential increase of on-chip computing
resources driven by Moore's Law for decades~\cite{mem-wall}.
Thus, the system performance is bound by the so-called memory wall.
The recent surge on highly data parallel and intensive applications
like video processing, dense DNN models, and signal processing makes
this issue even more serve --- a large portion of
the execution time and energy consumption is dominant
by moving the data back-and-forth
across memory hierarchies and computing units.
Many prior architectural solutions are proposed,
but few of them focus on a full-stack design.
Programming applications in low-level interfaces
not only limits the productivity of application development,
but also makes it hard to study the performance 
sensitivity of the applications under different
design decisions, because programs written in low-level
interfaces are often dedicated to a set of specific
design parameters.

Therefore, our goal is to build a full-stack, scalable, and
energy-efficient system that can effectively
specialize for the massive data parallelism among the applications.
We achieve this goal by presenting \sysname,
a full-stack bit-serial in-memory data processing system, and
Figure~\ref{fig:sys-overview} overviews it.

To productively develop applications with massive data parallelism
in a hardware-neutral way, we adopt
a tensor domain-specific language (DSL) as our high-level abstraction.
By taking advantage of both the domain knowledge provided by
tensor DSL and the underlying hardware's execution model,
the compiler can effectively find and distribute the 
parallelism and optimize the resource utilization
according to the given hardware parameters.

The underlying hardware is a multi-tile in-memory processing
system. Each tile has an imperative controller that commands
a cache with bit-serial computation enabled.
The bit-serial processing-in-memory (PIM) is attractive to us
because it not only enables massive data parallelism with intensive
computation resources at a modest hardware cost~\cite{ncache}
by adding logic units to each SRAM array, but also saves
significant energy and time to move data between caches and computing units.

Meanwhile, by connecting the tiles in a dynamically routed
on-chip network, the whole system can be flexibly scaled.
Having a larger on-chip cache allows fitting more data, which
also helps the throughput and latency.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/sys-overview.pdf}
    \caption{An overview to \sysname}
    \label{fig:sys-overview}
\end{figure}

\jian{I need a clearer way to talk about the three granularities of 
parallelism to get poised for the 2nd contribution.}

To sum up, the contributions of our framework are:
\begin{itemize}
    \item To the best of our knowledge, this work is the first one that studies the compilation techniques for bit-serial in-memory processing.
    \item A systematical tuning methodology to tune data parallelism distribution onto hardware specializations with different granularities.
    \item Cycle-accurate simulated performance characterization on a set of representative applications to determine the proper hardware design decision.
\end{itemize}


According to our evaluation, our compiler can achieve 
more than 95\% performance of expert-tuned kernels.
Our system can achieve 1.5x performance
on end-to-end DNN models over Nvidia A100
GPU, with only xx\% computational density
and yy\% energy consumption by saving zz\% DRAM-chip data traffic.

In the rest of the paper, we first discuss the backgrounds on
bit-serial in-memory processing and the tensor domain specific language in
Section~\ref{sec:bg}. We then overview the requirements and design decisions
of such a system in Section~\ref{sec:overview}. Then the compilation
techniques are elaborated in Section~\ref{sec:compiler}, and the
microarchitectures are discussed in Section~\ref{sec:uarch}
The techniques discussed before will be
evaluated \ref{sec:eval}, and the experiment setup will be
clarified in Section~\ref{sec:method}. Finally, we discuss related
work and conclude our work in Section~\ref{sec:rel} and \ref{sec:conc}.
